Survey on Additive Manufacturing, Cloud 3D Printing and Services

Cloud Manufacturing (CM) is the concept of using manufacturing resources in a service oriented way over the Internet. Recent developments in Additive Manufacturing (AM) are making it possible to utilise resources ad-hoc as replacement for traditional manufacturing resources in case of spontaneous problems in the established manufacturing processes. In order to be of use in these scenarios the AM resources must adhere to a strict principle of transparency and service composition in adherence to the Cloud Computing (CC) paradigm. With this review we provide an overview over CM, AM and relevant domains as well as present the historical development of scientific research in these fields, starting from 2002. Part of this work is also a meta-review on the domain to further detail its development and structure.

==> separated_figures/tab1.tex <==
\begin{table}
	\tbl{3D printing platforms and services included in this study -- Part 1}
	{\begin{tabular}[l]{llp{2.0cm}p{1.4cm}p{1.2cm}}
		\toprule
			Company/Service Name & URL & Classification & Established & Location\\
		\colrule
			3Faktur & \url{http://3faktur.com} & Modeling Service & 2014 & Germany \\
			3DaGoGo & \url{https://www.3dagogo.com} & Marketplace & 2013 & USA \\
			3DExport & \url{https://3dexport.com} & Marketplace, Repository & 2004 & USA \\
			3DHubs & \url{http://3dhubs.com} & Crowd Printing Provider & 2013 & USA \\
			3DPrinterOS & \url{https://www.3dprinteros.com} & Crowd Printing Provider & 2014 & USA \\
			3DShook & \url{http://www.3dshook.com} & Marketplace, Subscription Service & 2014 & Israel \\
			3D Warehouse & \url{https://3dwarehouse.sketchup.com} & Marketplace, Community, Repository & 2006 & USA \\
			Autodesk 123D & \url{http://www.123dapp.com} & Software, Marketplace, Repository & 2009 & USA \\
			Clara.io & \url{https://clara.io} & Repository, Modeling & 2013 & Canada \\
			CreateThis & \url{http://www.createthis.com} & Marketplace & 2013 & USA \\ 
			Cults & \url{https://cults3d.com} & Marketplace, Repository, Design Service & 2013 & France \\
			Grabcad & \url{https://grabcad.com} & Software, Marketplace, Repository & 2009 & USA \\
			La Poste & \url{http://impression3d.laposte.fr} & Print Provider, Marketplace & 2013 & France \\
			Libre3D & \url{http://libre3d.com} & Marketplace, Repository & 2014 & USA \\
			Makershop & \url{https://www.makershop.co} & Marketplace, Repository & 2013 & USA \\
			Materflow & \url{http://www.materflow.com} & Print Provider, Marketplace, Product Co-Creation/Support & 2013 & Finland \\
			MeltWerk & \url{https://www.meltwerk.com} & Print Provider & - & Subsidiary of trinckle \\
			MyMiniFactory & \url{https://www.myminifactory.com} & Crowd Printing Provider, Marketplace & 2013 & UK \\
					
			
			%\footnote{\url{https://www.theupsstore.com/about/pressroom/3d-printing-expands-across-the-nation}}
		\botrule
	\end{tabular}}
	%\tabnote{$^{\rm b}$This footnote shows the text turning over when a long footnote is added.}
	\label{tab:service_list}
\end{table}


==> separated_figures/tab2.tex <==
\begin{table}
	\tbl{3D printing platforms and services included in this study -- Part 2}
	{\begin{tabular}[l]{llp{2.0cm}p{1.4cm}p{1.2cm}}
		\toprule
			Company/Service Name & URL & Classification & Established & Location\\
		\colrule
			%3DXtras & \url{http://www.3dxtras.com} & Marketplace, Repository & Year & Loc \\
			NIH 3D Print Exchange & \url{http://3dprint.nih.gov} & Co-Creation, Repository & 2014 & USA \\
			p3d.in & \url{https://p3d.in} & Modeling & 2010 & Denmark \\
			Pinshape & \url{https://pinshape.com} & Marketplace & 2014 & Canada \\
			REPABLES & \url{http://repables.com} & Repository & 2013 & USA \\
			Rinkak & \url{https://www.rinkak.com} & Marketplace, Repository, Crowd Printing Provider & 2014 & Japan \\
			shapeking & \url{http://www.shapeking.com} & Marketplace, Repository & 2012 & Germany \\
			Shapetizer & \url{https://www.shapetizer.com} & Marketplace, Repository, Print Provider & 2015 & China \\
			Sketchfab & \url{https://sketchfab.com} & Marketplace, Repository & 2012 & France \\
			stlfinder & \url{http://www.stlfinder.com} & Search Engine & 2013 & Spain \\
			STLHive & \url{http://www.stlhive.com} & Marketplace, Repository, Design Service & 2015 & Canada \\
			Stratasys Direct Express & \url{https://express.stratasysdirect.com} & Print Provider & 2015 & USA \\
			Threeding & \url{https://www.threeding.com} & Marketplace, Print Provider & 2014 & Bulgaria \\
			Tinkercad & \url{https://www.tinkercad.com} & Design, Repository & 2011 & USA \\
			Treatstock & \url{https://www.treatstock.com} & Marketplace, Community, Crowd Printing Provider & 2016 & USA \\
			trinckle & \url{https://www.trinckle.com} & Print Provider & 2013 & Germany \\
			Trinpy & \url{https://www.trinpy.com} & Marketplace, Subscription Service & 2015 & Australia \\
			TurboSquid & \url{http://www.turbosquid.com} & Marketplace, Repository & 2000 & USA \\
			UPS & \url{https://www.theupsstore.com/print/3d-printing} & Print Provider & 2013 & USA \\			
			Watertight & \url{https://watertight.com} & Marketplace & 2015 & USA \\
			Yeggi & \url{http://www.yeggi.com} & Search Engine & 2013 & Germany \\
			YouMagine & \url{https://www.youmagine.com} & Community, Repository, Marketplace & 2013 & The Netherlands \\


		 % BL Lacs & 5 & 36 & 7 & $-4.0$ & $1.0\times 10^{-2}$ & 10$^\circ$ \\
		%  FSRQs & 5 & 40 & 11 & $-2.3$ & $0.5\times 10^{-2}$ & 14$^\circ$ \\
		\botrule
	\end{tabular}}
	%\tabnote{$^{\rm b}$This footnote shows the text turning over when a long footnote is added.}
	\label{tab:service_list_2}
\end{table}


==> separated_figures/tab3.tex <==
\begin{table}
	\tbl{3D printing platforms and services and their APIs - Part 1}
	{\begin{tabular}[l]{lp{1.4cm}p{1.4cm}p{1.4cm}p{1.4cm}c}
		\toprule
			Company / Service Name & Provides an API & Required for registration & Capabilities & Reach & Target Group\\
		\colrule
			3Faktur & No & N/A & N/A & Regional & Consumer \\
			3DaGoGo & No & N/A & N/A & Global & Consumer \\
			3DExport & No & N/A &  N/A & Global & Consumer + Professional \\
			3DHubs & Yes & Implementer + User & Upload & Global & Consumer \\
			3DPrinterOS & No & N/A & N/A & Global & Consumer \\
			3DPrintUK & No & N/A & Global & Consumer \\
			3DShook & No & N/A &  N/A & Global & Consumer \\
			3D Creation Lab & No & N/A & N/A & Global & Consumer \\
			3D Warehouse & No & N/A &  N/A & Global & Consumer \\
			Autodesk 123D & N/A &  No & N/A & Global & Consumer \\
			Clara.io & Yes & Implementer & Upload, Modify, Retrieve & Global & Consumer + Professional \\
			CreateThis & No & N/A &  N/A & Global & Consumer \\
			Cults & Yes (not public) & Implementer & View, Retrieve & Global & Consumer \\
			Grabcad & No & N/A & N/A & Global & Consumer + Professional\\
			iMakr & No & N/A & N/A & Global & Consumer \\
			i.Materialise & Yes & Implementer & Upload, Quoting, Order & Global & Consumer + Professional \\
			Kraftw\"urx.com & Yes (not public) & Implementer & Upload, Order & Global & Consumer \\
			La Poste & No & N/A & N/A & Regional & Consumer \\
			Libre3D & No & N/A &  N/A & Global & Consumer \\
			MakerBot / Thingiverse & Yes & Implementer & Upload, Retrieve & Global & Consumer \\
			Makershop & Yes & Implementer & Search, Retrieve & Global & Consumer + Professional \\
			MakeXYZ & Yes & Implementer + User & Order & Global & Consumer + Professional \\
			Materflow & No & N/A & N/A & Global & Consumer \\
			MeltWerk & Yes (not public) & Implementer & Upload, Quoting & Global & Consumer \\
			MyMiniFactory & No & N/A & N/A & Global & Consumer \\
			
		\botrule
	\end{tabular}}
	%\tabnote{$^{\rm b}$This footnote shows the text turning over when a long footnote is added.}
	\label{tab:service_api}
\end{table}


==> separated_figures/tab4.tex <==
\begin{table}
	\tbl{3D printing platforms and services and their APIs - Part 2}
	{\begin{tabular}[l]{lp{1.4cm}p{1.4cm}p{1.4cm}p{1.4cm}c}
		\toprule
			Company / Service Name & Provides an API & Required for registration & Capabilities & Reach & Target Group\\
		\colrule
			NIH 3D Print Exchange & Yes & Implementer & Upload, Retrieve & Global & Consumer \\
			p3d.in & No & N/A & N/A & Global & Consumer  \\
			Pinshape & No & N/A & N/A & Global & Consumer \\
			Ponoko & No & N/A & N/A & Global & Consumer \\
			REPABLES & No & N/A &  N/A & Global & Consumer \\
			Rinkak & Yes & Implementer & View, Order, Modeling & Global & Consumer \\
			Sculpteo & Yes & Implementer + User & Upload, Retrieve, Quoting, Order & Global & Consumer + Professional \\
			shapeking & No & N/A &  N/A & Global & Consumer \\
			Shapetizer & No N/A &  & N/A & Global & Consumer \\
			Shapeways & Yes & Implementer + User & Upload, Quoting, Order & Global & Consumer + Professional \\
			Sketchfab & Yes & Implementer & Upload, View & Global & Consumer \\
			stlfinder & No & N/A &  N/A & Global & Consumer \\
			STLHive & No & N/A &  N/A & Global & Consumer + Professional \\
			Stratsys Direct Express & No & N/A & N/A & Regional & Professional \\
			Threeding & No & N/A & N/A & Global & Consumer \\
			Tinkercad & No & N/A & N/A & Global & Consumer \\
			Treatstock & Yes & Implementer & Upload, Retrieve & Global & Consumer \\
			trinckle & No & N/A & N/A & Global & Consumer + Professional \\
			Trinpy & No & N/A &  N/A & Global & Consumer \\
			TurboSquid & No & N/A &  N/A & Global & Consumer + Professional \\
			UPS & No & N/A & N/A & Regional & Consumer \\
			Yeggi & Yes & Implementer & Search, Retrieve & Global & Consumer \\
			YouMagine & Yes & Implementer & Upload, Retrieve & Global & Consumer \\			
			Watertight & No & N/A & N/A & Global & Consumer \\
			
			%3DXtras & \url{http://www.3dxtras.com} & Marketplace, Repository & Year & Loc \\
		\botrule
	\end{tabular}}
	%\tabnote{$^{\rm b}$This footnote shows the text turning over when a long footnote is added.}
	\label{tab:service_api_2}
\end{table}


==> separated_figures/tab5.tex <==
\begin{table}
	\tbl{Categorising 3D printing online platforms}
	{\begin{tabular}[l]{p{2cm}|p{1.2cm}|p{1.4cm}|p{1.2cm}|p{1.4cm}|p{1.4cm}|p{1.2cm}|p{1.4cm}|p{1.4cm}l}
		\toprule
			Company / Service Name & Design market place & Design repository & Design service & Printing market place & Printing service & Printer sale & Crowd sourcing platform & Editor \\
		\colrule
			3Faktur & & & + & & + & & & \\
			3DaGoGo & + & + & & & & & & \\
			3DExport & + & + & & & & & & \\
			3DHubs & & & & + & + & & & \\
			3DPrinterOS & & & & + & + & & & \\
			3DPrintUK & & & + & & + & & & \\
			3DShook & + & + & & & & & & \\
			3D Creation Lab & & & & & + & & & \\
			3D Warehouse & + & + & & & & & & \\
			Autodesk 123D & + & + & & & + & & & \\
			Clara.io & + & + & & & & & & + \\
			CreateThis & + & + & & & & & & \\
			Cults & + & + & + & & & & & \\		
			Grabcad & + & + & & & & p & & + \\
			iMakr & & & & & + & + & & \\
			i.Materialise & + & + & + & & + & & + & \\
			Kraftw\"urx.com & + & + & + &  & + & & + & \\
			La Poste & + & + & & & + & & & + \\	
			Libre3D & + & + & & & & & & \\
			MakerBot / Thingiverse & + & + & & & & p & & + \\
			Makershop & + & + & & & & & & \\
			MakeXYZ & & & + & + & + & & & \\
			Materflow & + & + & + & & + & & & \\
			MeltWerk & & & & & + & & & \\
			MyMiniFactory & + & + & & & + & + & & \\
			NIH 3D Print Exchange & + & + & & & & & & \\
			p3d.in & + & + & & & & & & + \\
			Pinshape & + & + & & & & & & \\
			Ponoko & & & & & + & & & \\
			REPABLES & + & + & & & & & & \\
			Rinkak & + & + & & & + & & & \\
			Sculpteo & & & & & + & & & \\
			shapeking & + & + & & & & & & \\
			Shapetizer & + & + & & & + & & & \\
			Shapeways & + & + & & & + & & + & \\
			Sketchfab & + & + & & & & & & + \\
			stlfinder & & & & & & & & \\
			STLHive & + & + & + & & & & & \\
			Stratsys Direct Express & & & & & + & p & & \\
			Threeding & + & + & & & + & & & \\
			Tinkercad & + & + & & & o & & & + \\
			Treatstock & + & + & + & + & + & & & \\
			trinckle & & & & & + & & & \\
			Trinpy & + & + & & & & & & \\
			TurboSquid & + & + & & & & & & \\
			UPS & & & & & + & & & \\
			Watertight & + & + & & & & & & \\
			Yeggi & & & & + & + & & & \\
			YouMagine & + & + & & & o & p & & \\
			%3DXtras & \url{http://www.3dxtras.com} & Marketplace, Repository & Year & Loc \\
		\botrule
	\end{tabular}}
	%\tabnote{$^{\rm b}$This footnote shows the text turning over when a long footnote is added.}
	\label{tab:service_category}
\end{table}

